Construct 3D Hand Skeleton with Commercial WiFi

This paper presents HandFi, which constructs hand skeletons with practical WiFi devices. Unlike previous WiFi hand sensing systems that primarily employ predefined gestures for pattern matching, by constructing the hand skeleton, HandFi can enable a variety of downstream WiFi-based hand sensing applications in gaming, healthcare, and smart homes. Deriving the skeleton from WiFi signals is challenging, especially because the palm is a dominant reflector compared with fingers. HandFi develops a novel multi-task learning neural network with a series of customized loss functions to capture the low-level hand information from WiFi signals. During offline training, HandFi takes raw WiFi signals as input and uses the leap motion to provide supervision. During online use, only with commercial WiFi, HandFi is capable of producing 2D hand masks as well as 3D hand poses. We demonstrate that HandFi can serve as a foundation model to enable developers to build various applications such as finger tracking and sign language recognition, and outperform existing WiFi-based solutions. Artifacts can be found: https://github.com/SIJIEJI/HandFi

==> discussion.tex <==
\section{Discussion}
% \textcolor{blue}{\paragraph{Potential Downstream Applications.}}
% \textcolor{blue}{In addition to freeing the system from the constraints of a predefined set of gestures, allowing more flexible and convenient extensions for gesture recognition, the ability of HandFi to directly model the skeleton of the hand provides many new possibilities for downstream tasks. We enumerate some potential applications: 1. Privacy-preserving biometric authentication: hand shape (the width of the palm and the length of the hand) and the skeleton (bone length and palm structure) together can be used as a unique biometric authentication to enable personal identification in a convenient and privacy-preserving way. 2. Advanced gaming and immersive experiences: The ability to function in the dark could offer a more interactive and immersive gameplay experience. 3. Health Monitoring: The ability to capture subtle hand motions such as hand tremors could be indicative of conditions such as Parkinson's disease or anxiety disorders. It can also be used to help monitor patients recovering from hand injuries in a user-friendly way. 4. Smart retail: personalized shopping experience based on the unique hand movements of customers, interactive advertising on the shelf, and contactless payments. 5. Education: Virtual musical instrument training, such as playing piano.}




